Clustering with missing data: which imputation model for which cluster analysis method?

Multiple imputation (MI) is a popular method for dealing with missing values. One main advantage of MI is to separate the imputation phase and the analysis one. However, both are related since they are based on distribution assumptions that have to be consistent. This point is well known as congeniality. In this paper, we discuss congeniality for clustering on continuous data. First, we theoretically highlight how two joint modeling (JM) MI methods (JM-GL and JM-DP) are congenial with various clustering methods. Then, we propose a new fully conditional specification (FCS) MI method with the same theoretical properties as JM-GL. Finally, we extend this FCS MI method to account for more complex distributions. Based on an extensive simulation study, all MI methods are compared for various cluster analysis methods (k-means, k-medoids, mixture model, hierarchical clustering). This study highlights the partition accuracy is improved when the imputation model accounts for clustered individuals. From this point of view, standard MI methods ignoring such a structure should be avoided. JM-GL and JM-DP should be recommended when data are distributed according to a gaussian mixture model, while FCS methods outperform JM ones on more complex data.

==> algo_FCS_homo.tex <==
Denoting $[\bfA,\bfB]$ the matrix obtained by merging two matrices $\bfA$ and $\bfB$ on the rows, $\bfZ_\nbvar^{obs}$ the column $\nbvar$ of $\bfZ$ restricted to its $\Nbind_\nbvar^{obs}$ observed observations (i.e. so that $r_{\nbind\nbvar}=1$ with $\sum_\nbind \left(r_{\nbind\nbvar}\right) =\Nbind_\nbvar^{obs}$), $\bfZ_{-\nbvar}$ the set of continuous variables except column $\nbvar$ and $\bfZ_{-\nbvar}^{obs}$ the set restricted to observed observations on $\bfZ_\nbvar$, the proposed algorithm is as follows:
\begin{enumerate}
    \item Initialization:  
    \begin{itemize}
        \item Using the EM algorithm, find the ML estimate of $\bfzeta$ and initialize $\bfW^{(0)}$ by a draw from the posterior distribution and ${\bfZ^{miss}}^{(0)}$ by a draw from its posterior distribution given $\bfW^{(0)}$
    \end{itemize}
    \item for $\nbiter$ in $\{1,...,\Nbiter\}$
    \begin{enumerate}
    \item $\bfZ\leftarrow \bfZ^{(\nbiter-1)}$
    \item for $\nbvar$ in \{$1,...,\Nbvar\}$
    \begin{enumerate}
        \item \label{eqnquanti}draw $\bfbeta_\nbvar^\star$ and $\sigma_\nbvar^\star$ (the parameters of the linear regression model used to impute the $\nbvar$th variable) from their posterior distribution \citep{VB18}:
        \begin{itemize}
            \item fit the ML estimators $\left(\widehat{\bfbeta}_\nbvar,\widehat{\sigma}_\nbvar\right)$ of the linear regression model $Z_\nbvar^{obs}=\left[\bfU^{(\nbiter-1)}\bfZ_{-\nbvar}\right]^{obs}\bfbeta_\nbvar+\varepsilon$ with $\varepsilon\sim\mathcal{N}\left(0,\sigma^2I_{\Nbind_\nbvar^{obs}}\right)$ 
            \item draw $df$ from $\chi^2(\Nbind_\nbvar^{obs}-\Nbvar-\Nbgroup+1)$ and compute $\sigma_\nbvar^{\star^2}=\left(\hat{\varepsilon}\right)^t\hat{\varepsilon}/df$
            \item draw $\bfbeta_\nbvar^\star$ from \begin{equation} \mathcal{N}\left(\widehat{\bfbeta}_\nbvar,\sigma_\nbvar^{\star^2} \left(\left(\left[\bfU^{(\nbiter-1)}\bfZ_{-\nbvar}^{obs}\right]\right)^t\left[\bfU^{(\nbiter-1)}\bfZ_{-\nbvar}^{obs}\right]\right)^{-1}\right)
            \end{equation}
        \end{itemize}
        \item \label{eqnquanti2}impute the missing values of ${\bfZ_{\nbvar}}$ from  $\mathcal{N}\left(\left[\bfU^{(\nbiter-1)}\bfZ_{-\nbvar}\right]^{miss}\bfbeta_\nbvar^{\star},{\sigma_\nbvar^\star}^2I_{\Nbind_\nbvar^{miss}}\right)$
    \end{enumerate}
    \item $\bfZ^{(\nbiter)}\leftarrow \bfZ$
    \item \label{eqnquali1} by resampling individuals, generate a bootstrap replication $\bfZ^\star$ from $\bfZ^{(\ell)}$ and estimate $\bfzeta$ the set of parameters of a homoscedastic gaussian mixture model. The associated estimate is denoted $\bfzeta^\star$ 
    \item draw $w_\nbind^\star$ (for all $1\leq\nbind\leq\Nbind$) from
    \begin{equation}\label{eqnhomo1}
       P(W=w)\propto exp\left(\left({\bfmu^{\star}_\nbgroup}\right)^t\left(\bfSigma^{\star}\right)^{-1}\bfz_\nbind
    -\frac{1}{2}\left(\bfmu^{\star}_\nbgroup\right)^t\left({\bfSigma^{\star}}\right)^{-1}{\bfmu^{\star}_\nbgroup}+log(\bftheta^{\star}_\nbgroup)\right)
    \end{equation} and derive the disjunctive table $\bfU^{\star}$
    \item draw $\bftheta^{(\nbiter)}$ from $\mathcal{D}\left(\alpha+diag\left(\left(\bfU^{\star}\right)^t\bfU^{\star}\right)\right)$
    \item draw $w^{(\nbiter)}_\nbind$ (for all $1\leq\nbind\leq\Nbind$) from 
    \begin{equation}\label{eqnhomo2}
       P(W=w)\propto exp\left(\left({\bfmu^{\star}_\nbgroup}\right)^t\left(\bfSigma^{\star}\right)^{-1}\bfz_\nbind
    -\frac{1}{2}\left(\bfmu^{\star}_\nbgroup\right)^t\left(\bfSigma^{\star}\right)^{-1}{\bfmu^{\star}_\nbgroup}+log(\bftheta^{(\nbiter)}_\nbgroup)\right)
    \end{equation}
    \end{enumerate}
\end{enumerate}

==> frogicu.tex <==
\subsection{FROG-ICU}
\VA{copier-coller... : FROG-ICU was a prospective, observational, multicenter cohort study of intensive care unit (ICU)  survivors followed 1 year after discharge, including 21 medical, surgical or mixed ICUs in France and Belgium. All consecutive patients admitted to intensive care with a requirement for invasive mechanical ventilation and/or vasoactive drug support for more than 24 h following ICU admission and discharged from ICU were included. Clinical and biological parameters on ICU discharge were measured, including the circulating cardiovascular biomarkers N-terminal pro-B type natriuretic peptide, high-sensitive troponin I, bioactive-adrenomedullin and soluble-ST2.}

The FROG-ICU study gathers $\Nbind = $ \VA{à compléter} patients, which can be classified in 3 groups according to their septic shocks: \VA{detailler}. Septic shocks are generally diagnosed from clinical parameters. For our purpose, we aims at looking the three clusters from $\Nbvar = $ \VA{à compléter} biomarkers.

==> titleabstractkeywords.tex <==
\maketitle

\textbf{Abstract} Multiple imputation (MI) is a popular method for dealing with missing values. One main advantage of MI is to separate the imputation phase and the analysis one. However, both are related since they are based on distribution assumptions that have to be consistent. This point is well known as \textit{congeniality}.

In this paper, we discuss congeniality for clustering on continuous data. First, we theoretically highlight how two joint modeling (JM) MI methods (JM-GL and JM-DP) %by the general location model or based on the Dirichlet process mixture of products of multivariate normal distributions
are congenial with various clustering methods. Then, we propose a new fully conditional specification (FCS) MI method with the same theoretical properties as JM-GL. Finally, we extend this FCS MI method to account for more complex distributions. Based on an extensive simulation study, all MI methods are compared for various cluster analysis methods (k-means, k-medoids, mixture model, hierarchical clustering).

This study highlights the partition accuracy is improved when the imputation model accounts for clustered individuals. From this point of view, standard MI methods ignoring such a structure should be avoided. JM-GL and JM-DP should be recommended when data are distributed according to a gaussian mixture model, while FCS methods outperform JM ones on more complex data.

\vspace{1cm}

\textbf{Keywords}: Clustering; Missing Data; Multiple imputation; Congeniality.

==> wine.tex <==
\subsection{Wine data set}
The wine data set \citep{wine} is considered to illustrate the flexibility of FCS MI methods compared to JM MI methods for clustering. Such a data set describes $\Nbind=178$ Italian wines by $\Nbvar=13$ chemical descriptors. These wines can be clustered in $\Nbgroup=3$ categories (corresponding to 3 cultivars). Since the data set is full, 40\% missing values are added according to a MCAR or a MAR mechanism (as described in Section \ref{secdatagen}). 100 missing data patterns are considered for each mechanism.

JM MI methods are applied using the same parameters as those described in Section \ref{misim}. For FCS MI methods, variable selection is performed from each incomplete data to define each conditional imputation model. The method used is fully described in \citet{Barhen20}, it consists in repeating imputation and variable selection on subset of variables drawn at random. On each subset, imputation is performed using JM-GL and variable selection using knockoff \citep{Barber15}. %(see Tables \ref{varselwine} and \ref{varselwine_mar} in Appendix for details about the imputation models used). 
 The number of clusters is set to $\Nbgroup=3$ for the proposed FCS MI methods. In practice, it could be estimated from incomplete values according to Equation \ref{nbdegroup}.% (see Appendix \ref{nbgroupwine} for results). 
The number of iterations is tuned to $\Nbiter=200$.% Continuous variables are imputed by predictive mean matching for FCS-homo.

After multiple imputation ($\Nbtab=20$), cluster analysis is performed using Gaussian mixture model (with constraint of equal volume and shape but variable orientation on the covariance matrices), k-means clustering, partitioning around medoids and hierarchical clustering. ARI are reported in Figure \ref{fig:real}. %is reported in Table \ref{tab:real}, while the cluster instability (obtained from Equation \ref{B3}) is reported in Table \ref{tab:inst}.

\begin{figure}[H]
   \centering
    \includegraphics[scale=.5]{Figures/res.real.simu.pdf}
    \caption{Wine data set: adjusted rand index (ARI) over 100 missing data patterns for various MI methods (FCS-homo, FCS-hetero, FCS-norm, JM-DP, JM-GL and JM-norm) and various cluster analysis methods (mixture, partitioning around medoids, hierarchical clustering, k means) on the incomplete wine data set. Two missing data patterns are investigated: a pattern from a MCAR mechanism (on the top) and one from a MAR mechanism (on the bottom). In both cases, 40\% of values are missing. Results for JM-GL and JM-norm are missing under the MCAR mechanism because of failures of the MI methods.}
   \label{fig:real}
\end{figure}

Because the number of variables is relatively large according to the number of observations, some imputation methods (JM-GL and JM-norm) cannot be generally applied. On the contrary, by specifying conditional imputation models, FCS methods are less subject to this issue. Furthermore, according to the ARI, FCS-homo outperforms others imputation models under the MCAR mechanism. Under the MAR mechanism, the advantage of this method is less evident, but it remains among the imputation methods providing the partition with the highest ARI for all cluster analysis methods.

%\begin{figure}[H]
%    \centering
%    \includegraphics[scale=.35]{resreal.pdf}
%     \includegraphics[scale=.35]{resrealmar.pdf}
%    \caption{Wine data set: adjusted rand index (ARI) for various MI methods (FCS-homo, FCS-hetero, FCS-norm, JM-DP, JM-GL and JM-norm) and various cluster analysis methods (mixture, partitioning around medoids, hierarchical clustering, k means) on the incomplete wine data set. Two missing data patterns are investigated: a pattern from a MCAR mechanism (on the left) and one from a MAR mechanism (on the right). In both cases, 40\% of values are missing. Some results are missing because of failures of the MI methods.}
%    \label{fig:real}
%\end{figure}

%\begin{table}[ht]
%\centering
%\tiny
%\caption{Wine data set: adjusted rand index (ARI) for various MI methods (FCS-homo, FCS-hetero, FCS-norm, JM-DP, JM-GL and JM-norm) and various cluster analysis methods (mixture, partitioning around medoids, hierarchical clustering, k means) on the incomplete wine data set. Two missing data patterns are investigated: a pattern from a MCAR mechanism  and one from a MAR mechanism. In both cases, 40\% of values are missing. Some results are missing because of failures of the MI methods. The highest ARI are printed in boldface. \label{tab:real}}
%\begin{tabular}{rllrrrrrr}
%  \hline
% & mech & analysis & JM-DP & JM-GL & JM-norm & FCS-hetero & FCS-homo & FCS-norm \\ 
%  \hline
%1 & mcar & mixture & 0.816 & 0.701 &  & 0.815 & \textbf{0.864} & 0.815 \\ 
%  2 & mcar & pam & 0.741 & 0.770 &  & \textbf{0.815} & 0.771 & 0.740 \\ 
%  3 & mcar & cah & 0.755 & 0.686 &  & \textbf{0.799} & 0.788 & 0.769 \\ 
%  4 & mcar & kmeans & 0.756 & 0.755 &  & \textbf{0.831} & 0.801 & 0.754 \\ 
%  5 & mar & mixture & 0.743 & 0.619 & 0.731 & \textbf{0.773} & 0.673 & 0.729 \\ 
%  6 & mar & pam & 0.702 & 0.690 & 0.674 & \textbf{0.775} & 0.715 & 0.678 \\ 
%  7 & mar & cah & 0.732 & 0.729 & 0.746 & \textbf{0.773} & 0.700 & 0.717 \\ 
%  8 & mar & kmeans & 0.737 & 0.703 & 0.762 & \textbf{0.773} & 0.762 & 0.748 \\ 
%   \hline
%\end{tabular}
%\begin{tabular}{ll|p{.3cm}|p{.3cm}|p{.3cm}|rr|rrrr|rrrr}
% \hline
%  mech & analysis &\multicolumn{13}{c}{imputation method} \\\hline
%& & JM-DP & JM-GL & JM-norm & \multicolumn{2}{c}{FCS-hetero}  & \multicolumn{4}{c}{FCS-homo}  & \multicolumn{4}{c}{FCS-norm}
%\\ &&&&&all&select& \multicolumn{2}{c}{all}& \multicolumn{2}{c}{select}& \multicolumn{2}{c}{all}& \multicolumn{2}{c}{select}
%\\  &&&&&&&norm&pmm&norm&pmm&norm&pmm&norm&pmm \\\hline
%mcar & mixture & 0.82 & 0.70 &  &  & 0.79 & 0.77 & 0.80 & 0.83 & 0.83 & 0.85 & 0.83 & 0.71 & 0.78 \\ 
%  mcar & pam & 0.74 & 0.77 &  &  & 0.80 & 0.73 & 0.76 & 0.77 & 0.78 & 0.76 & 0.74 & 0.74 & 0.73 \\ 
%  mcar & hc & 0.75 & 0.69 &  &  & 0.83 & 0.80 & 0.76 & 0.80 & 0.78 & 0.77 & 0.82 & 0.70 & 0.73 \\ 
%  mcar & kmeans & 0.76 & 0.75 &  &  & 0.82 & 0.77 & 0.80 & 0.77 & 0.78 & 0.78 & 0.77 & 0.76 & 0.73 \\ 
%  mar & mixture & 0.74 & 0.62 & 0.73 & 0.75 & 0.74 & 0.70 & 0.72 & 0.71 & 0.73 & 0.73 & 0.74 & 0.73 & 0.80 \\ 
%  mar & pam & 0.70 & 0.69 & 0.67 & 0.70 & 0.76 & 0.70 & 0.72 & 0.72 & 0.73 & 0.75 & 0.69 & 0.69 & 0.78 \\ 
%  mar & hc & 0.73 & 0.73 & 0.75 & 0.71 & 0.77 & 0.70 & 0.71 & 0.72 & 0.75 & 0.74 & 0.77 & 0.72 & 0.75 \\ 
%  mar & kmeans & 0.74 & 0.70 & 0.76 & 0.73 & 0.77 & 0.70 & 0.74 & 0.72 & 0.76 & 0.76 & 0.78 & 0.71 & 0.78 \\ 
%   \hline
%\end{tabular}
%\end{table}

%To make interpretation of ARI easier, an analysis of the variance is used to explain the ARI according to the imputation model, the analysis model, the missing data mechanism as well as the interaction between the imputation model and the analysis one. Results are reported in Tables \ref{Ftest} and \ref{Ttest}.

%As observed on the simulation study, the ARI is sensitive to the imputation method used (p value = 0.001), while  the cluster analysis method considered does not modify the ARI (p value = 0.156). Table \ref{Ttest} shows higher ARI are obtained with FCS MI methods (highest estimates for FCS-homo or FCS-hetero among effects related to the imputation method). Furthermore, among FCS methods (resp. JM method), heteroscedastic imputation models generally outperform homoscedastic models. \MRR{Avons nous une explication? C'est quand même plutot l'inverse dans les autres simulations? Est ce que les distributions des \emph{winemarker} sont gaussiennes?}\VA{oui, plutôt}

%\begin{table}[ht]
%\centering
%\caption{ANOVA table summarizing global effects of the cluster analysis method, the imputation model, the mechanism and the interaction between the analysis model and the imputation model on the ARI \label{Ftest}}
%\begin{tabular}{p{4cm}rrrrr}
%  \hline
% & SS & df & MS & F value & Pr($>$F) \\ 
%  \hline
%cluster analysis & 0.006 & 3 & 0.002 & 1.95 & 0.1560 \\ 
%  imputation model & 0.032 & 5 & 0.006 & 6.37 & 0.0012 \\ 
%  mechanism & 0.029 & 1 & 0.029 & 28.59 & 0.0000 \\ 
%  interaction clus:imp & 0.016 & 15 & 0.001 & 1.07 & 0.4409 \\ 
%  residuals & 0.019 & 19 & 0.001 &  &  \\ 
%   \hline
%\end{tabular}
%\end{table}
% latex table generated in R 4.0.3 by xtable 1.8-4 package
% Wed Feb 17 18:37:36 2021
%\begin{table}[ht]
%\centering
%\caption{ANOVA table summarizing local effects of the imputation model and the mechanism on the ARI (sum to zero contrasts is used).\label{Ttest}}
%\begin{tabular}{rrrrr}
%  \hline
% & Estimate & Std. Error & $t$ value & Pr($>|t|$) \\ 
%  \hline
%(Intercept) & 0.7510 & 0.0052 & 144.66 & 0.00 \\ 
%  imp - FCS-hetero & 0.0432 & 0.0108 & 4.00 & 0.00 \\ 
%  imp - FCS-homo & 0.0082 & 0.0108 & 0.76 & 0.45 \\ 
%  imp - FCS-norm & -0.0072 & 0.0108 & -0.66 & 0.51 \\ 
%  imp - JM-DP & -0.0033 & 0.0108 & -0.31 & 0.76 \\ 
%  imp - JM-GL & -0.0447 & 0.0108 & -4.14 & 0.00 \\ 
%  imp - JM-norm & 0.0038 & 0.0150 & 0.25 & 0.80 \\ 
%  mech - mar & -0.0268 & 0.0052 & -5.17 & 0.00 \\ 
%  mech - mcar & 0.0268 & 0.0052 & 5.17 & 0.00 \\ 
%   \hline
%\end{tabular}
%\end{table}

%As regard partition instability, homoscedastic imputation methods (JM-GL and FCS-homo) provide more stable partitions than heteroscedastic imputation methods (FCS-hetero, JM-DP). FCS-norm and JM-DP provide the most instable partitions, meaning clusters are more difficult to identify. Indeed, while other imputation methods used the true number of clusters, both make different assumptions: FCS-norm assumes individuals are not clustered, while JM-DP allows the number of clusters varies between 1 and 5. By this way, the first method makes difficult to identify the cluster structure after imputation, making the final partition instable; while the second have the same behavior if one or two clusters are considered and tends to increase the variability of imputed values when this number is equal to 4 or 5.
%\begin{table}[H]
%\centering \caption{Instability of the clustering procedure under a MCAR or a MAR mechanism: 5 imputation methods are investigated (FCS-homo, FCS-hetero, FCS-norm, JM-DP or JM-GL) using $\Nbtab=20$ imputed data sets and several cluster analyses methods (mixture, pam, k-means, hierarchical clustering).\label{tab:inst}}
%\begin{tabular}{rlrrrrr}
%  \hline
% & mech & FCS-hetero & FCS-homo & FCS-norm & JM-DP & JM-GL \\ 
%  \hline
%mixture & mcar & 0.35 & 0.26 & 0.46 & 0.49 &  \\ 
%  pam & mcar & 0.26 & 0.22 & 0.31 & 0.34 & 0.15 \\ 
%  hc & mcar & 0.24 & 0.21 & 0.35 & 0.36 & 0.14 \\ 
%  kmeans & mcar & 0.16 & 0.13 & 0.19 & 0.23 & 0.09 \\ \hline \hline
%  mixture & mar & 0.28 & 0.24 & 0.32 & 0.43 & 0.20 \\ 
%  pam & mar & 0.22 & 0.18 & 0.22 & 0.29 & 0.18 \\ 
%  hc & mar & 0.24 & 0.18 & 0.26 & 0.34 & 0.17 \\ 
%  kmeans & mar & 0.13 & 0.11 & 0.13 & 0.18 & 0.09 \\ 
%   \hline
%\end{tabular}
%\end{table}
